Measurements of ZZ production with the ATLAS detector and simulation of loop-induced processes with the HERWIG event generator

This thesis presents results and method developments in both experimental and theoretical particle physics. The main part shows measurements of $\ell^+\ell^-\ell'^+\ell'^-$ production (where $\ell$, $\ell'$ is either an electron or a muon) in proton-proton collisions at 13 TeV centre-of-mass energy. The collisions were produced by the Large Hadron Collider in 2015 and 2016 and observed with the ATLAS detector. In a phase space sensitive to Z boson pair production, the integrated cross section as well as differential cross sections with respect to twenty-one observables are measured. Ten of these directly measure associated jet activity. The measurements provide an important test of the Standard Model of particle physics. A direct search for effects beyond the Standard Model affecting ZZ production is performed in a generic effective field theory approach. No significant deviations from the Standard Model predictions are observed. Exclusion limits are set on the parameters describing new physics in the effective field theory. In theoretical developments, the automated description of loop-induced processes with the Herwig 7 event generator is presented. These are processes that can only occur via a quantum loop of virtual particles. Preliminary results in leading-order quantum chromodynamics are shown for the production of a Higgs boson, of a pair of Higgs bosons, and of four leptons. The Higgs boson results show that the full loop-induced description can deviate significantly from the common approximation where the mass of the top quark is treated as infinitely large. Thus, including loop effects is crucial to obtaining precise predictions to compare to measurements at the Large Hadron Collider. Developments towards a next-to-leading-order description of arbitrary loop-induced processes are shown.

==> Final_CombinedCorrelationMatrix_fourLepton_mass_binning0.tex <==
\begin{tabular}{lrrrrrrrrrrrrrr}
\toprule
$m_{4\ell}$ [GeV] &  140--180 &  180--200 &  200--220 &  220--240 &  240--260 &  260--280 &  280--300 &  300--325 &  325--350 &  350--400 &  400--500 &  500--600 &  600--800 &  800--1500 \\
\midrule
140--180  &      1.00 &      0.44 &     -0.29 &     -0.17 &     -0.16 &     -0.06 &     -0.23 &     -0.10 &     -0.25 &     -0.18 &     -0.03 &      0.10 &      0.11 &       0.04 \\
180--200  &      0.44 &      1.00 &     -0.10 &     -0.06 &     -0.02 &      0.02 &     -0.11 &     -0.02 &     -0.10 &     -0.06 &      0.03 &      0.08 &      0.07 &       0.05 \\
200--220  &     -0.29 &     -0.10 &      1.00 &      0.16 &      0.10 &      0.06 &      0.16 &      0.10 &      0.13 &      0.10 &      0.08 &      0.02 &      0.02 &       0.03 \\
220--240  &     -0.17 &     -0.06 &      0.16 &      1.00 &      0.14 &      0.04 &      0.11 &      0.10 &      0.12 &      0.08 &      0.09 &      0.01 &      0.02 &      -0.01 \\
240--260  &     -0.16 &     -0.02 &      0.10 &      0.14 &      1.00 &      0.12 &      0.07 &      0.02 &      0.15 &      0.10 &      0.06 &      0.04 &      0.05 &      -0.01 \\
260--280  &     -0.06 &      0.02 &      0.06 &      0.04 &      0.12 &      1.00 &      0.13 &     -0.01 &      0.09 &     -0.01 &      0.05 &      0.06 &      0.04 &       0.01 \\
280--300  &     -0.23 &     -0.11 &      0.16 &      0.11 &      0.07 &      0.13 &      1.00 &      0.11 &      0.04 &      0.06 &      0.07 &     -0.02 &      0.01 &       0.05 \\
300--325  &     -0.10 &     -0.02 &      0.10 &      0.10 &      0.02 &     -0.01 &      0.11 &      1.00 &      0.10 &      0.05 &      0.03 &      0.01 &      0.06 &      -0.00 \\
325--350  &     -0.25 &     -0.10 &      0.13 &      0.12 &      0.15 &      0.09 &      0.04 &      0.10 &      1.00 &      0.08 &      0.03 &      0.01 &      0.02 &       0.01 \\
350--400  &     -0.18 &     -0.06 &      0.10 &      0.08 &      0.10 &     -0.01 &      0.06 &      0.05 &      0.08 &      1.00 &      0.02 &     -0.01 &      0.00 &       0.03 \\
400--500  &     -0.03 &      0.03 &      0.08 &      0.09 &      0.06 &      0.05 &      0.07 &      0.03 &      0.03 &      0.02 &      1.00 &     -0.03 &     -0.02 &       0.01 \\
500--600  &      0.10 &      0.08 &      0.02 &      0.01 &      0.04 &      0.06 &     -0.02 &      0.01 &      0.01 &     -0.01 &     -0.03 &      1.00 &      0.03 &       0.02 \\
600--800  &      0.11 &      0.07 &      0.02 &      0.02 &      0.05 &      0.04 &      0.01 &      0.06 &      0.02 &      0.00 &     -0.02 &      0.03 &      1.00 &      -0.04 \\
800--1500 &      0.04 &      0.05 &      0.03 &     -0.01 &     -0.01 &      0.01 &      0.05 &     -0.00 &      0.01 &      0.03 &      0.01 &      0.02 &     -0.04 &       1.00 \\
\bottomrule
\end{tabular}


==> Final_StatCorrelationMatrix_fourLepton_mass_binning0.tex <==
\begin{tabular}{lrrrrrrrrrrrrrr}
\toprule
$m_{4\ell}$ [GeV] &  140--180 &  180--200 &  200--220 &  220--240 &  240--260 &  260--280 &  280--300 &  300--325 &  325--350 &  350--400 &  400--500 &  500--600 &  600--800 &  800--1500 \\
\midrule
140--180  &      1.00 &      0.07 &     -0.10 &      0.02 &      0.03 &     -0.03 &     -0.04 &      0.01 &      0.01 &      0.02 &      0.02 &      0.00 &      0.01 &      -0.00 \\
180--200  &      0.07 &      1.00 &     -0.04 &     -0.03 &      0.01 &      0.00 &     -0.06 &      0.00 &     -0.01 &     -0.01 &      0.01 &     -0.00 &     -0.01 &       0.01 \\
200--220  &     -0.10 &     -0.04 &      1.00 &      0.01 &     -0.05 &     -0.04 &      0.01 &      0.01 &     -0.02 &     -0.03 &      0.00 &      0.01 &      0.01 &       0.01 \\
220--240  &      0.02 &     -0.03 &      0.01 &      1.00 &      0.01 &     -0.04 &     -0.01 &      0.03 &     -0.00 &     -0.03 &      0.02 &     -0.02 &      0.00 &      -0.03 \\
240--260  &      0.03 &      0.01 &     -0.05 &      0.01 &      1.00 &      0.04 &     -0.05 &     -0.06 &      0.04 &     -0.00 &     -0.01 &      0.01 &      0.02 &      -0.03 \\
260--280  &     -0.03 &      0.00 &     -0.04 &     -0.04 &      0.04 &      1.00 &      0.07 &     -0.06 &      0.02 &     -0.07 &      0.00 &      0.03 &      0.01 &      -0.01 \\
280--300  &     -0.04 &     -0.06 &      0.01 &     -0.01 &     -0.05 &      0.07 &      1.00 &      0.04 &     -0.09 &     -0.04 &      0.00 &     -0.04 &     -0.00 &       0.02 \\
300--325  &      0.01 &      0.00 &      0.01 &      0.03 &     -0.06 &     -0.06 &      0.04 &      1.00 &      0.04 &     -0.01 &     -0.01 &     -0.00 &      0.05 &      -0.02 \\
325--350  &      0.01 &     -0.01 &     -0.02 &     -0.00 &      0.04 &      0.02 &     -0.09 &      0.04 &      1.00 &     -0.02 &     -0.02 &      0.00 &      0.02 &      -0.00 \\
350--400  &      0.02 &     -0.01 &     -0.03 &     -0.03 &     -0.00 &     -0.07 &     -0.04 &     -0.01 &     -0.02 &      1.00 &     -0.04 &     -0.02 &     -0.01 &       0.02 \\
400--500  &      0.02 &      0.01 &      0.00 &      0.02 &     -0.01 &      0.00 &      0.00 &     -0.01 &     -0.02 &     -0.04 &      1.00 &     -0.06 &     -0.05 &      -0.01 \\
500--600  &      0.00 &     -0.00 &      0.01 &     -0.02 &      0.01 &      0.03 &     -0.04 &     -0.00 &      0.00 &     -0.02 &     -0.06 &      1.00 &     -0.01 &      -0.02 \\
600--800  &      0.01 &     -0.01 &      0.01 &      0.00 &      0.02 &      0.01 &     -0.00 &      0.05 &      0.02 &     -0.01 &     -0.05 &     -0.01 &      1.00 &      -0.06 \\
800--1500 &     -0.00 &      0.01 &      0.01 &     -0.03 &     -0.03 &     -0.01 &      0.02 &     -0.02 &     -0.00 &      0.02 &     -0.01 &     -0.02 &     -0.06 &       1.00 \\
\bottomrule
\end{tabular}

